Transpiling Quantum Circuits using the Pentagon Equation

We consider the application of the pentagon equation in the context of quantum circuit compression. We show that if solutions to the pentagon equation are found, one can transpile a circuit involving non-Heisenberg-type interactions to a circuit involving only Heisenberg-type interactions while, in parallel, reducing the depth of a circuit. In this context, we consider a model of non-local two-qubit operations of Zhang \emph{et. al.} (the $A$ gate), and show that for certain parameters it is a solution of the pentagon equation.

==> letter.tex <==

To the Editors of Phys. Rev. A 

We would like to submit the attached manuscript entitled “Transpiling Quantum Circuits using the Pentagon Equation” for consideration for publication in Phys. Rev. A.

Our submission can be seen in two ways. First, it offers a useful clarification on the recent paper of Bo et al. (``Quantum time dynamics employing the Yang-Baxter equation for circuit compression'', Phys. Rev. A 106, 012412,  published 8 July 2022), where we show that the only solution of the Yang-Baxter equation is actually not particularly useful in circuit compression, as the circuit would have to use multiple identity gates in order for the circuit compression using the Yang-Baxter equation to apply. 

In addition to the corrective function above, our paper also considers a closely related, so-called Pentagon equation, which can be used in a similar fashion to the Yang-Baxter equation. 

Finally, it develops a notion of local/non-local duality. ...
